Trust Me If You Can: Trusted Transformation Between (JSON) Schemas to Support Global Authentication of Education Credentials

Recruiters and institutions around the world struggle with the verification of diplomas issued in a diverse and global education setting. Firstly, it is a nontrivial problem to identify bogus institutions selling education credentials. While institutions are often accredited by qualified authorities on a regional level, there is no global authority fulfilling this task. Secondly, many different data schemas are used to encode education credentials, which represents a considerable challenge to automated processing. Consequently, significant manual effort is required to verify credentials. In this paper, we tackle these challenges by introducing a decentralized and open system to automatically verify the legitimacy of issuers and interpret credentials in unknown schemas. We do so by enabling participants to publish transformation information, which enables verifiers to transform credentials into their preferred schema. Due to the lack of a global root of trust, we utilize a distributed ledger to build a decentralized web of trust, which verifiers can query to gather information on the trustworthiness of issuing institutions and to establish trust in transformation information. Going beyond diploma fraud, our system can be generalized to tackle the generalized problem for other domains lacking a root of trust and agreements on data schemas.

==> figures/graph1.tex <==
\begin{figure}[h]
    \centering
    \begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=4cm,thick,
                        wot node/.style={circle,draw,font=\bfseries, fill=yellow!10,minimum size=2cm},
                        t node/.style={circle,draw,font=\bfseries, fill=yellow!10,minimum size=2cm}]
    
      \node[wot node] (2) {Uni B};
      \node[wot node] (1) [below left of=2] {Uni A};
      \node[wot node] (3) [below right of=2] {Uni C};
      
      \node[t node] (5) [below left of=3] {Schema Y};
      \node[t node] (4) [below left of=5] {Schema X};
      \node[t node] (6) [below right of=5] {Schema Z};
    
      \path
        (1) 
        edge node [left] {} (2)
        
        (2) 
        %edge [bend right] node [left] {$e_{B \rightarrow A}$} (1)
        edge node [right] {} (3)
        
        %(4) 
        %edge node [left] {$e_{FB \rightarrow B}$} (2)
        %edge node [above] {$e_{FB \rightarrow FC}$} (5)
       ;      
       
       
       \path
        (4) 
        edge node [left] {} (5)
        
        (5) 
        %edge [bend right] node [left] {$e_{B \rightarrow A}$} (1)
        edge node [right] {} (6)
        
        %(4) 
        %edge node [left] {$e_{FB \rightarrow B}$} (2)
        %edge node [above] {$e_{FB \rightarrow FC}$} (5)
       ;    
    \end{tikzpicture}
    \caption{Example graphs and IPFS.}
    \label{fig:graph1}
\end{figure}

==> figures/solidity-highlighting.tex <==
% Copyright 2017 Sergei Tikhomirov, MIT License
% https://github.com/s-tikhomirov/solidity-latex-highlighting/

%\usepackage{listings, xcolor}

\definecolor{verylightgray}{rgb}{.97,.97,.97}

\lstdefinelanguage{Solidity}{
	keywords=[1]{anonymous, assembly, assert, balance, break, call, callcode, case, catch, class, constant, continue, constructor, contract, debugger, default, delegatecall, delete, do, else, emit, event, experimental, export, external, false, finally, for, function, gas, if, implements, import, in, indexed, instanceof, interface, internal, is, length, library, log0, log1, log2, log3, log4, memory, modifier, new, payable, pragma, private, protected, public, pure, push, require, return, returns, revert, selfdestruct, send, solidity, storage, struct, suicide, super, switch, then, this, throw, transfer, true, try, typeof, using, value, view, while, with, addmod, ecrecover, keccak256, mulmod, ripemd160, sha256, sha3}, % generic keywords including crypto operations
	keywordstyle=[1]\color{blue}\bfseries,
	keywords=[2]{address, bool, byte, bytes, bytes1, bytes2, bytes3, bytes4, bytes5, bytes6, bytes7, bytes8, bytes9, bytes10, bytes11, bytes12, bytes13, bytes14, bytes15, bytes16, bytes17, bytes18, bytes19, bytes20, bytes21, bytes22, bytes23, bytes24, bytes25, bytes26, bytes27, bytes28, bytes29, bytes30, bytes31, bytes32, enum, int, int8, int16, int24, int32, int40, int48, int56, int64, int72, int80, int88, int96, int104, int112, int120, int128, int136, int144, int152, int160, int168, int176, int184, int192, int200, int208, int216, int224, int232, int240, int248, int256, mapping, string, uint, uint8, uint16, uint24, uint32, uint40, uint48, uint56, uint64, uint72, uint80, uint88, uint96, uint104, uint112, uint120, uint128, uint136, uint144, uint152, uint160, uint168, uint176, uint184, uint192, uint200, uint208, uint216, uint224, uint232, uint240, uint248, uint256, var, void, ether, finney, szabo, wei, days, hours, minutes, seconds, weeks, years},	% types; money and time units
	keywordstyle=[2]\color{teal}\bfseries,
	keywords=[3]{block, blockhash, coinbase, difficulty, gaslimit, number, timestamp, msg, data, gas, sender, sig, value, now, tx, gasprice, origin},	% environment variables
	keywordstyle=[3]\color{violet}\bfseries,
	identifierstyle=\color{black},
	sensitive=false,
	comment=[l]{//},
	morecomment=[s]{/*}{*/},
	commentstyle=\color{gray}\ttfamily,
	stringstyle=\color{red}\ttfamily,
	morestring=[b]',
	morestring=[b]"
}

\lstset{
	language=Solidity,
	backgroundcolor=\color{verylightgray},
	%extendedchars=true,
	basicstyle=\footnotesize\ttfamily,
	showstringspaces=false,
	showspaces=false,
	numbers=none,
	%numberstyle=\footnotesize,
	%numbersep=9pt,
	tabsize=2,
	%breaklines=true,
	showtabs=false,
	%captionpos=b
}


==> meta/introduction-old.tex <==
\section{Introduction}
% TODO: more selling, more references with motivation
% TODO: make sure use of certificate/credential/diploma is consistent


\todoi{cite Rome Communiqué?}
% https://github.com/Knowledge-Innovation-Centre/HEIDI/blob/master/HEIDI%20Mission%20Statement.md#f1

\todoi{F1: highlight impact, compare costs with paper-based}

\todoi{M: arguments about seriousness of issue (e.g. study how many fake creds, etc?)}

\todoi{M: erwähnen, welche uni schon digitale credentials hat, ... dadurch ermöglicht unser system dass bestehende sachen practical werden}

When an international \student applies to study at a university abroad or for a job, they need to document past education achievements.
Similarly, if a \student completes courses at a different university (e.\,g.\ during a study mobility program) or in an online course, certificates of the course grades are required for the course to be recognized at the \student's home university.
To prove their accomplishments, \students provide education evidence, e.\,g.\ a graduation diploma or similar prerequisite for university entrance.
Such a diploma contains information about the \student and the achieved degree as well as information identifying the institution issuing the \credential.
Additionally, information like a stamp and signatures are added to help verify the diploma's authenticity.
Since achieving a university degree is time-consuming and often expensive, some people take a shortcut and buy their diploma at a fake university, a so-called diploma mill~\cite{Littlefield2020,Noble1998,Contreras2009,Noble1998a,DepartmentEducation2009}.
Others simply fake their diploma outright~\cite{Jr2004}.
\citet{Borresen2020} identify three categories of fake \credentials:
(a) \capitalCredentials that look as if they were issued by a legitimate university, while in fact they were not.
(b) \capitalCredentials that were actually issued by a legitimate university, but modified afterwards by the \student, e.\,g.\ by improving grades or graduation level.
(c) \capitalCredentials that were issued by universities that do not exist or exist for the sole purpose of selling fake diplomas.
% In a paper world this typically done by forging signatures or stamps on fake or stolen document paper, and by altering the documents.
According to the UK's Department of Education, 240 universities were identified as fake universities in 2020 in the UK alone \cite{UDE2020}.
Correspondingly, education systems and universities invest a lot of effort towards the validation of \credentials to ensure they are legitimate~\cite{Borresen2020}.
% TODO: more numbers from the sources in ``Detecting Fake University Degrees in a Digital World''
\todoi{TODO: a few sentences about how paper credentials are verified currently (various institutions, paper documents in original, attestations by lawyer/embassy, ...)}
\todoi{mention databases like Nuffic and Anabin, maybe IMI (ETER, HEDD are mentioned in next paragraph, though)}

In an increasingly digitized world, graduation diplomas can also be represented as digital documents in the form of \credentials.
\todoi{1-2 sentences about digital diplomas/relwork here already?}

To reduce or even eliminate the risk of accepting fake \credentials or \credentials issued by a diploma mill, universities need to verify \credentials, including the authenticity and legitimacy of the \credential's issuer.
While fakes of categories (a) and (b) are easy to detect if \credentials are signed using digital signatures, (c) involves expensive checks even in a digital setting.
% On one hand, verifying that a respective \issuer issued a credential can easily be done using digital signatures.
% On the other hand, it is a non-trivial task to ensure the \issuer is actually authorized to issues a certain credential.
Verification of legitimacy could be done by checking lists provided by the respective governments, but such lists are rarely available.
Not all countries publish the list of recognized educational institutions in a machine-readable format, and even if they do so, they often do not include all information required for verification (such as public keys)~\cite{UDE2020,OfficeStudents2018,ETERConsortium2020}.
\todoi{ref ETER, HEDD, US, ...}
Furthermore, ``legitimate university'' means different things in different countries and contexts, putting the burden on universities to decide on and enforce their own regulations.
% Thus, a different approach is needed.

\todoi{mention DAFI, TestAS as credential supplement/substitute?}

When verifying \credentials issued by an educational institution in a different country or education system, an additional problem arises:
On the one hand, issuing digital \credentials in a machine-readable format requires the issuing institution to decide on the format and schema it uses to encode the diploma information.
This diploma needs to fulfill various requirements depending on the context, such as the structure of the education system, content of a course or study, and legal regulations.
On the other hand, the institution trying to verify such \credentials needs to understand the formats and schemata used therein.
Thus the \issuer and \verifier have to not only agree on file formats, but also on the schema to represent the \credential data, which is a challenge on its own.


\subsection{Challenges}

\todoi{F3: remove overlap with prev section (→ merge)}

In our increasingly globalized and digitized education world, there is currently still no system which can be used to automatically authenticate education evidence, such as diplomas, grades and other \credentials.
While most institutions are able to perform those authentications in a manual way (checking paper-based forms, demanding notarization or an apostille, consulting lawyers, etc.), this process needs to be repeated for every \credential and every \issuer.
In addition, an institution needs to perform the full authentication for a \credential even if a (trusted) partner institution already previously verified this \credential.
The same is true for the opposite case, i.\,e.\ when a partner institution identifies a \issuer as fake.
This is an unnecessary duplication of effort, since authentication processes for \credentials are always the same (even though final approval depends on the verifying institution's policies and regulations).

% TODO: make clearer that the system is used to assist, not to fully authenticate (which poses more legal issues).

To assist a university's study service center or HR department, and to reduce the effort needed to authenticate education \credentials, a document/degree verification system needs to perform the following checks:

\begin{itemize}
    \item collect information about the identity and legitimacy of the issuing university based on \verifier's regulations;
    \item verify that a \credential was really issued by this university, and that it was not altered;
    \item transfer the \credential into a schema known to the \verifier; and
    \item perform further checks based on the content of the \credential w.\,r.\,t.\ local regulations.
\end{itemize}


\subsection{Contribution}

% TODO: terminology cleanup

\todoi{think about level of detail here, e.g. mention that institutions are represented by DID, \credentials are VCs, etc.?}

\todoi{F4: highlight generic usecase, not just edu}

\todoi{generalize storage, only mention IPFS in impl}

In this paper we introduce a trust management system based on distributed ledger (DL) technology.
The properties provided by DLs and its use for academic \credentials have been positively evaluated before~\cite{Grech2017}, but the problem of evaluating the legitimacy of \issuers in a global setting remains.
We use a DL to enable all institutions involved to publish trust information about \issuers, effectively forming a web of trust (WoT).
% The idea is to use a distributed-ledger as storage for a web of trust.
A web of trust is a directed graph of trust information:
The vertices in this graph represent educational institutions (or possibly other stakeholders) while the edges represent trust information about the legitimacy of an \issuer.
All institutions are able to publish outgoing edges from their own vertex, thus adding information about whom they trust to be legitimate -- or, conversely, whom they believe to be illegitimate.
This information is encoded as set of tuples containing information on how much they trust the other entity. % and how they verified the identity.
This allows a \verifier to define their own rules on how to classify and categorise the trust in a (previously unknown) institution.
% An incoming edge basically represents a certification similar to a certificate in PKI, thus confirming that the vertex indeed represents the DID of a certain entity.

Since an edge can also carry a negative trust statement, it is important that no entity has the power to delete or hide an edge.
We achieve this by using a decentralized data structure in a smart contract.

While other trust management systems focus on the question of \textit{ensuring that a certain identifier indeed belongs to an entity}, or system is more concerned with the question of whether \textit{a certain identifier represents a legitimate credential issuer}.

In addition to publishing trust information about the legitimacy of an \issuer, a second graph contains information on how to transform the \credential from the \student's schema into a schema known to the \verifier.

This information is then retrieved by a \verifier and used to authenticate \issuers, and to automatically process the \credentials based on rules locally defined in a trust policy.

In \Cref{sec:concept} we explain this concepts in more detail.

Additionally, we provide a reference implementation which uses a Solidity smart contract on an Ethereum-based DL to store the graphs and IPFS to store \transInfo.
We also introduce a simple system based on JSON templates allowing for transformation of a JSON document from one schema into another.
More details about our implementation are given in \Cref{sec:impl}, wherein we show that our approach is feasible.
Furthermore, we discuss some our concept's properties and theoretical features in \Cref{sec:discuss}.

\todoi{arguments why we need a DL (central location but not governed by one party, availability, proof of nonexistence of a negative edge, ...}

\todoi{make clear trust path from \verifier to \issuer needs to be complete (no trust in certifications from fake \certifiers, etc.)}

\todoi{M: highlight novelty, e.g. we combine established technique A and B to achieve novel properties C}

%\missingfigure{arch overview figure, WoT with transformations?}


==> protocol1.tex <==
\newcommand{\marginfix}{0.4em}

\begin{table*}[th!]
		\caption{Protocol Phases}
	\label{tab:protocol}
	\begin{tabular}{|p{8.5cm}|p{8.5cm}|}
		\hline

		\multicolumn{2}{|l|}{\textbf{General Parameters:} Our protocol relies on a digital signature scheme \SIG, a Distributed Ledger \DL, and \IPFS.}\\

		\hline

		\begin{description}[leftmargin=\marginfix]
            %\setlength{\parskip}{0.5em}

			\item[\pSetup:]~
			\begin{itemize}[label={},leftmargin=\marginfix]
				\item \on{any \capitalCreator}
				\begin{enumerate}
					\item Generate key pair $(\pk_\any, \sk_\any) \gets \KeyGen()$ 
                    
                    \item Create smart contract for WoT registry
                    
                    \item Use key pair to install smart contract at \DL on address $\Acontract$
                    
                    %\item delete key pair
                    
                    \item Announce address $\Acontract$ and contract code (out-of-band)
				\end{enumerate}

				\item \on{all \capitalStudent{}s, \capitalIssuer{}s, and \capitalCertifier{}s}
				\begin{enumerate}[resume]
				    \item Generate key pair $(\pk, \sk) \gets \KeyGen()$ 
                    \item Create $\DID$ from $\pk$ and use it to register $\pk$ at \DL
				\end{enumerate}
            
			\end{itemize} %end: Setup
			
			\vspace{0.5em}

			\item[\pIssueCert:]~
			\begin{itemize}[label={},leftmargin=\marginfix]
				\item \on{\capitalCertifier $\Certifier$}
				\begin{enumerate}
				    \item Verify identity and legitimacy of issuer, and obtain issuer's $\DID_\Issuer$ (out-of-band, e.g., via existing social networks)

                    \item Create the WoT edge $\edge$, which includes 
                    \begin{enumerate}
                    \item the \certifier's~$\DID_\Certifier$,
                    \item the issuer's~$\DID_\Issuer$,
                    \item the attested level of legitimacy as issuer~$\level$,
                    \item the attested level of confidence as \certifier~$\confidence$,
                    \item the certification's context $\context$ set to \textit{credential},
                    \item the type $\uri$ to a URI identifying a \credential type, and
                    \item the current time $\timeSymbol$
                    \end{enumerate}
                    
                    %\item create the transformation edge $\edge$, which includes 
                    %the Certifier's~$\DID_\Certifier$ ,
                    %the certification Issuer's~$\DID_\Issuer$ ,
                    %the attested level of trust in the transformation~$\level$,
                    %the attested level of confidence as transformation %publisher~$\confidence$,
                    %the certification's context $\context$ set to \textit{transformation},
                    %and the current time t
                    
                    \item Sign the edge: $\sigma_\edge \gets \SIG.\Sign(\edge, \sk_\Certifier)$
                    
                    \item Add signature as additional attribute to edge $\edge$, yielding~$\edge'$
                    
                    \item Send edge to contract: $\DL.\DLCall(\Acontract, \SCaddWOT, \edge')$
				\end{enumerate}
            
                \item \on{all \DL nodes}
                \begin{enumerate}[resume]
                    \item Receive the \certifier's request to add the edge $\edge'$
                    
                    %\item verifiy that the caller's DID corrosponds to $\DID_\Certifier$\newline
                    %in the given edge
                    
                    \item Add $\edge'$ to the WoT graph's list of edges
                    %, overwriting other edges with same $(\DID_\Certifier, \DID_\Issuer)$ pair
                \end{enumerate}
                
                \item\vspace{0.3em}\hspace{-0.8em}\underline{Revoke \capitalCertificate:} can be achieved as in Phase \numIssueCert, but with different values for the levels $\level$ and $\confidence$
            
			\end{itemize} %end: Certification
		\end{description} 
    &
		\begin{description}[leftmargin=\marginfix]
            %\setlength{\parskip}{0.5em}
            
            
			\item[\pIssueCred:]~
			\begin{itemize}[label={},leftmargin=\marginfix]
			    \item \on{\capitalStudent $\Student$}
				\begin{enumerate}
				    \item Request verifiable \credential by authenticating with university, and send their~$\DID_\Student$ as well as proof of ownership of~$\sk_\Student$ 
				\end{enumerate}

				\item \on{\capitalIssuer $\Issuer$}
				\begin{enumerate}[resume]
					\item Verify \student's identity and ownership of~$\DID_\Student$
                    
                    %\item verify student's ownership of~$\DID_\Student$
                    
                    \item Encode the \student's attributes~$A_\Student$ using~$\schema_\Issuer$, yielding~$A_\Student'$
                    
                    \item Generate the verifiable \credential~$\cred$, which includes the encoded attributes~$A_\Student'$ , the \student's~$\DID_\Student$, and the issuer's~$\DID_\Issuer$ 
                    
                    \item Sign the \credential $\sigma_{\cred} \gets \SIG.\Sign(\cred, \sk_\Issuer)$, \newline
                    and add~$\sigma_{\cred}$ to~$\cred$, yielding~$\cred'$
                    
                    \item Issue the signed \credential~$\cred'$ to the \student
				\end{enumerate}
            
			\end{itemize} %end: Issuing

            \vspace{0.5em}

			\item[\pVerify:]~
			\begin{itemize}[label={},leftmargin=\marginfix]
		
				\item \on{\capitalStudent $\Student$}
				\begin{enumerate}
				    \item Send $\DID_\Student$, proof of ownership of $\sk_\Student$ and $\cred'$ to the \verifier
                    %\item provide $\cred$ to Verifier 
				\end{enumerate}

				\item \on{\capitalVerifier $\Verifier$}
				\begin{enumerate}[resume]
					
                    \item Load up-to-date WoT graph from \DL: \newline
                    $\wot \gets \DL.\DLCall(\Acontract, \SCgetWOT)$
                    
                    %\item load credential revocation status from \DL \newline
                    %$\revoc \leftarrow \DL.\DLCall(\Arevoc, \SCget, \id_{\cred})$
                    
                    %\item verify that $\revoc$ contains a valid status
                    
                    \item Load issuer's public key from \DL:\newline
                    $\pk_\Issuer \gets \DL.\DLResolve(\DID_\Issuer)$,
                    where $\DID_\Issuer$ from $\cred'$
                    
                    \item Verify that issuer was not revoked/expired and allowed to issue while issuing
                    
                    \item Verify that \credential was really signed by that issuer 
                    $\SIG.\Verify(\cred', \pk_\Issuer) = 1$
                    
                    \item Find paths from \verifier to issuer relevant w.r.t. $\cred'$ \newline
                     $\paths \gets \pathfinder(\wot, \DID_\Verifier, \DID_{\Issuer}, \context_{\cred'}, \uri_{\cred'})$
                     
                    \item Authenticate edges in $\paths$ by verifying its $\sigma_\edge$\newline
                     $\forall \vpath \in \paths, \forall \vedge~\edge \in \vpath: \SIG.\Verify(\edge, \pk_\Certifier) = 1$, \newline
                    % $\land  \pk_{\Certifier_\vedge} = \DL.\DLResolve(\cred_{\DID_\Issuer})$
                    where $\DID_\Certifier$ from $\vedge~\edge$ and $\pk_\Certifier \gets \DL.\DLResolve(\DID_\Certifier)$

                    \item Compute overall legitimacy of issuer and verify it w.r.t. \policy:                    $\calcscore(\paths) \geq \policy_{\minscore}$
                    
				\end{enumerate}
			\end{itemize}\vspace{-1em} %end: Verification
		\end{description} \\ \hline
		
		\begin{description}[leftmargin=\marginfix]
			\item[\pIssueTrans:]~
			\begin{itemize}[label={},leftmargin=\marginfix]
				\item \on{\capitalCertifier $\Certifier$}
				\begin{enumerate}
                    \item Define transformation information~$\transl_{X \rightarrow Y}$ from~$\schema_X$ to~$\schema_Y$,
                    and publish it on~$\IPFS$ on address~$\Atranslation$ 
                    
                    \item Create the transformation edge $\edge_T$, which includes 
                    \begin{enumerate}
                        \item the \certifier's~$\DID_\Certifier$,
                        \item the URI identifying the source schema $\schema_X$,
                        \item the URI identifying the target schema $\schema_Y$,
                        \item the IPFS address of the transformation~$\Atranslation$, and
                        \item the current time $\timeSymbol$
                    \end{enumerate}
                    
                    \item Sign the edge $\sigma_{\edge_{\Ttrans}} \gets \SIG.\Sign(\edge_T, \sk_\Certifier)$
                    
                    \item Add the signature as additional attribute to the transformation edge, yielding~$\edge_\Ttrans'$
                    
                    \item Send edge to contract $\DL.\DLCall(\Acontract, \SCaddT, \edge_\Ttrans')$
				\end{enumerate}
            
                \item \on{all \DL nodes}
                \begin{enumerate}[resume]
                    % \item Receive the \certifier's requests to add the edge to the transformation graph
                    
                    %\item verifiy that the caller's DID corrosponds to $\DID_\Certifier$\newline
                    %in the given edge
                    
                    \item Add $\edge_\Ttrans'$ to the transformation graph's list of edges
                    %, overwriting other edges with same $(\DID_\Certifier, \DID_\Issuer)$ pair
                \end{enumerate}
                
                \item\vspace{0.3em}\hspace{-0.8em}\underline{\pIssueTCert:} can be achieved as in Phase (2), but with 
                the certification's context $\context$ set to \textit{transformation},
                and the identifier $\uri$ to a URI identifying a \credential schema.
            
			\end{itemize}\vspace{-1em} %end
		\end{description}
    &
		\begin{description}[leftmargin=\marginfix]

			\item[\pVerifyTrans:]~
			\begin{itemize}[label={},leftmargin=\marginfix]
				\item \on{\capitalVerifier $\Verifier$}
				\begin{enumerate}
                    %\item[] \textit{(optional)} transform $\cred$ to $\schema_\Verifier$ and verify policy:
                    
                    \item Load up to date transformation graph from \DL \newline
                    $\transf \gets \DL.\DLCall(\Acontract, \SCgetT)$
                    
                    \item Find paths from issuer's to \verifier's schema \newline
                     $\paths_\Ttrans \gets \pathfinder(\transf, \schema_\Issuer, \schema_\Verifier)$
                    
                    \item For each $\vpath$ in $\paths_\Ttrans$:
                    \begin{enumerate}[leftmargin=1em]
                            \item $\cred' \gets \cred$
                            
                            \item For each $\vedge$ in $\vpath$:
                             \begin{enumerate}[leftmargin=1em]
                                 \item Authenticate $\vedge$ by using $\wot$
                                % TODO: explain this^ in more detail?
                                
                                 %\item verify that $\confidence_\edge$ is higher than $\policy_{\minconf}$
                                 
                                 \item Get transformation address~$\Atranslation$ from edge
                                 
                                 \item Load transformation~$\transl \gets \IPFS.\load(\Atranslation)$
                                 
                                 \item Transform \credential~$\cred' \gets \translate(\transl, \cred')$
                             \end{enumerate}
                         
                             \item Verify that $\cred'$ fulfills $\policy_{\rules}$ or reject with reason 
                            %   if not reject $\cred'$ with reason why
                    \end{enumerate}
                    
                    \item Accept $\cred$ for further human processing
                    
                    % \item interact with $n$ nodes to seal $\DID_\Prover$, i.e. \newline
                    % $\forall i \in [n]: \sigma_i \gets \MSIG.\Sign(\DID_\Prover, \sk_i) $ and\newline
                    % $\sigma_{\DID_\Prover} \gets \MSIG.\ASigs(\{(\pk_i, \sigma_i)\}_{\forall i \in [n]})$
                    % \item issue $\sigma_{\DID_\Prover}$ to the user
                    % \todo[inline]{also generate seal on public key of DID, so that this can be forwarded when offline}
				\end{enumerate}
            
			\end{itemize}\vspace{-1em} %end: Verification
		\end{description}\\
		\hline
	\end{tabular} \\
\vspace*{-2em}
\end{table*}



